An Investigation of the Test-Retest Reliability of the miniPXI

Repeated measurements of player experience are crucial in games user research, assessing how different designs evolve over time. However, this necessitates lightweight measurement instruments that are fit for the purpose. In this study, we conduct an examination of the test-retest reliability of the \emph{miniPXI} -- a short variant of the \emph{Player Experience Inventory} (\emph{PXI}), an established measure for measuring player experience. We analyzed test-retest reliability by leveraging four games involving 100 participants, comparing it with four established multi-item measures and single-item indicators such as the Net Promoter Score (\emph{NPS}) and overall enjoyment. The findings show mixed outcomes; the \emph{miniPXI} demonstrated varying levels of test-retest reliability. Some constructs showed good to moderate reliability, while others were less consistent. On the other hand, multi-item measures exhibited moderate to good test-retest reliability, demonstrating their effectiveness in measuring player experiences over time. Additionally, the employed single-item indicators (\emph{NPS} and overall enjoyment) demonstrated good reliability. The results of our study highlight the complexity of player experience evaluations over time, utilizing single and multiple items per construct measures. We conclude that single-item measures may not be appropriate for long-term investigations of more complex PX dimensions and provide practical considerations for the applicability of such measures in repeated measurements.

==> table_master.tex <==
\afterpage{%
\begin{landscape}
\begin{table}
\centering
\small
\setlength{\tabcolsep}{2.0pt}
\def\arraystretch{0.86}
\caption{Mean and standard deviations ($SD$) across week 1 and 3, Intra-class correlation coefficient (ICC) interpretation in terms of test-retest reliability (
$0.25 \leq ICC < 0.5$: poor = \textcolor{cPoor}{\rule{2.5ex}{1.5ex}}; $0.5 \leq ICC < 0.75$: moderate = \textcolor{cModerate}{\rule{2.5ex}{1.5ex}}; $0.75 \leq ICC < 0.9$: good = \textcolor{cGood}{\rule{2.5ex}{1.5ex}}; $ICC \geq 0.9$: excellent = \textcolor{cExcellent}{\rule{2.5ex}{1.5ex}}), 95\% confidence interval (CI), reliability analysis (Cronbach’s $\alpha$, and McDonald’s $\omega$) for multiple-item measures across week 1 and 3, for each construct.}
\vskip-0.5\baselineskip
\label{table:all_questionnaires}

\begin{tabularx}{1.0\linewidth}{ll c cc@{\hskip10pt} cc@{\hskip10pt} d{2.3}cccc@{\hskip12pt}  d{2.3}cc@{\hskip12pt} cccc@{\hskip12pt} cccc}
\toprule

&  &  &  &  &  & & \multicolumn{5}{c}{\textbf{Mean difference}} & \multicolumn{3}{c}{\hskip-6pt\textbf{Cohen's} $\bm{d}$} & \multicolumn{4}{c}{\textbf{Int. Consistency}} & \multicolumn{3}{c}{\textbf{T-RT Reliability}} \\

\cmidrule(lr){8-12} \cmidrule(lr){13-15} \cmidrule(lr){16-19} \cmidrule(lr){20-22}

&  & & \multicolumn{2}{c}{\textbf{Mean (SD)}} &  &  &  &   & \multicolumn{2}{c}{\textbf{95\% CI}} &  &  & \multicolumn{2}{c}{\hskip-6pt\textbf{95\% CI}} & \multicolumn{2}{c}{\textbf{Week 1}} & \multicolumn{2}{c}{\textbf{Week 3}} &  & \multicolumn{2}{c}{\textbf{95\% CI}} \\

\cmidrule(lr){4-5} \cmidrule(lr){10-11} \cmidrule(lr){14-15} \cmidrule(lr){21-22}

& \textbf{Construct} & \textbf{\#I} & \textbf{Week 1} & \textbf{Week} 3 & \textbf{NRMSE} & \textbf{MAD} & \multicolumn{1}{c}{$\bm{\Delta}$\textbf{Mean}} & $\bm{\Delta}$\textbf{SE} & \textbf{L} & \textbf{U} & $\bm{p}$ & \multicolumn{1}{c}{$\bm{d}$} & \textbf{L} & \textbf{U} & $\bm{\alpha}$ & $\bm{\omega}$ & $\bm{\alpha}$ & $\bm{\omega}$ & \textbf{ICC} & \textbf{L} & \textbf{U} \\

\midrule
\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textbf{miniPXI}}}}
& Audiovisual Appeal    & 1     & 5.65 (1.35) & 5.69 (1.35) & 0.20 & 0.72 &  -0.04 & 0.12 & -0.27 & 0.19 & 0.732 & -0.03 & -0.23 & 0.16 & - & - & - & - & \icc{0.630} & 0.496 & 0.735 \\
& Challenge             & 1     & 4.80 (1.51) & 5.12 (1.53) & 0.34 & 1.14 &  -0.32 & 0.16 & -0.64 & 0.00 & 0.052 & -0.20 & -0.39 & 0.00 & - & - & - & - & \icc{0.422} & 0.249 & 0.570 \\
& Ease of Control       & 1     & 6.01 (1.38) & 6.06 (1.16) & 0.22 & 0.71 &  -0.05 & 0.13 & -0.31 & 0.21 & 0.703 & -0.04 & -0.23 & 0.16 & - & - & - & - & \icc{0.479} & 0.312 & 0.617 \\
& Clarity of Goals      & 1     & 5.72 (1.61) & 5.77 (1.51) & 0.23 & 0.75 &  -0.05 & 0.14 & -0.32 & 0.22 & 0.714 & -0.04 & -0.23 & 0.16 & - & - & - & - & \icc{0.624} & 0.488 & 0.731 \\
& Progress Feedback     & 1     & 5.11 (1.61) & 5.00 (1.75) & 0.27 & 0.95 &   0.11 & 0.14 & -0.17 & 0.39 & 0.436 &  0.08 & -0.12 & 0.27 & - & - & - & - & \icc{0.651} & 0.522 & 0.751 \\
& Autonomy              & 1     & 5.32 (1.50) & 5.12 (1.47) & 0.28 & 1.06 &   0.20 & 0.15 & -0.09 & 0.49 & 0.179 &  0.14 & -0.06 & 0.33 & - & - & - & - & \icc{0.505} & 0.345 & 0.637 \\
& Curiosity             & 1     & 5.64 (1.24) & 5.69 (1.40) & 0.22 & 0.77 &  -0.05 & 0.13 & -0.30 & 0.20 & 0.692 & -0.04 & -0.24 & 0.16 & - & - & - & - & \icc{0.547} & 0.393 & 0.671 \\
& Immersion             & 1     & 6.19 (1.10) & 6.07 (1.17) & 0.21 & 0.70 &   0.12 & 0.13 & -0.13 & 0.37 & 0.351 &  0.09 & -0.10 & 0.29 & - & - & - & - & \icc{0.365} & 0.183 & 0.523 \\
& Mastery               & 1     & 5.43 (1.43) & 5.43 (1.22) & 0.26 & 0.96 &   0.00 & 0.14 & -0.28 & 0.28 & 1.000 &  0.00 & -0.20 & 0.20 & - & - & - & - & \icc{0.447} & 0.274 & 0.591 \\
& Meaning               & 1     & 4.72 (1.49) & 4.72 (1.53) & 0.27 & 0.86 &   0.00 & 0.13 & -0.25 & 0.25 & 1.000 &  0.00 & -0.20 & 0.20 & - & - & - & - & \icc{0.644} & 0.513 & 0.746 \\
& Enjoyment             & 1     & 5.88 (1.24) & 5.88 (1.26) & 0.16 & 0.50 &   0.00 & 0.10 & -0.19 & 0.19 & 1.000 &  0.00 & -0.20 & 0.20 & - & - & - & - & \icc{0.704} & 0.590 & 0.791 \\
 
\midrule
\multicolumn{2}{l}{\textbf{NPS}} & 1     & 6.21 (2.65) & 6.29 (2.74) & 0.28 & 1.18 &  -0.08 & 0.18 & -0.43 & 0.27 & 0.649 & -0.05 & -0.24 & 0.15 & - & - & - & - & \icc{0.791} & 0.704 & 0.854 \\

\midrule
\multicolumn{2}{l}{\textbf{Appreciation}}  & 1     & 5.70 (1.28) & 5.73 (1.25) & 0.14 & 0.45 &  -0.03 & 0.08 & -0.19 & 0.13 & 0.712 & -0.04 & -0.23 & 0.16 & - & - & - & - & \icc{0.795} & 0.710 & 0.857 \\

\midrule
\parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textbf{PXI}}}}
& Audiovisual Appeal    & 3     & 5.92 (1.00) & 5.92 (0.90) & 0.13 & 0.45 &   0.00 & 0.16 & -0.33 & 0.33 & 1.000 &  0.00 & -0.39 & 0.39 & 0.95 & 0.96 & 0.94 & 0.94 & \icc{0.668} & 0.374 & 0.840 \\
& Challenge             & 3     & 5.12 (1.37) & 5.03 (1.23) & 0.15 & 0.63 &   0.09 & 0.16 & -0.23 & 0.42 & 0.561 &  0.12 & -0.28 & 0.51 & 0.88 & 0.88 & 0.80 & 0.81 & \icc{0.820} & 0.634 & 0.916 \\
& Ease of Control       & 3     & 6.08 (1.00) & 6.20 (0.71) & 0.12 & 0.52 &  -0.12 & 0.15 & -0.42 & 0.18 & 0.424 & -0.16 & -0.56 & 0.23 & 0.90 & 0.91 & 0.78 & 0.81 & \icc{0.643} & 0.341 & 0.825 \\
& Clarity of Goals      & 3     & 5.88 (1.03) & 5.72 (1.01) & 0.09 & 0.40 &   0.16 & 0.11 & -0.06 & 0.38 & 0.149 &  0.30 & -0.11 & 0.70 & 0.89 & 0.90 & 0.89 & 0.89 & \icc{0.856} & 0.701 & 0.934 \\
& Progress Feedback     & 3     & 5.41 (1.26) & 5.53 (1.48) & 0.20 & 0.89 &  -0.12 & 0.23 & -0.59 & 0.35 & 0.602 & -0.11 & -0.50 & 0.29 & 0.88 & 0.89 & 0.90 & 0.90 & \icc{0.664} & 0.370 & 0.837 \\
& Autonomy              & 3     & 5.05 (1.37) & 5.04 (1.32) & 0.22 & 0.79 &   0.01 & 0.23 & -0.45 & 0.48 & 0.953 &  0.01 & -0.38 & 0.40 & 0.91 & 0.91 & 0.91 & 0.91 & \icc{0.657} & 0.356 & 0.833 \\
& Curiosity             & 3     & 6.04 (0.67) & 5.87 (1.07) & 0.14 & 0.44 &   0.17 & 0.18 & -0.20 & 0.54 & 0.344 &  0.19 & -0.20 & 0.59 & 0.90 & 0.91 & 0.94 & 0.94 & \icc{0.495} & 0.137 & 0.740 \\
& Immersion             & 3     & 5.77 (0.87) & 5.65 (1.13) & 0.13 & 0.47 &   0.12 & 0.15 & -0.18 & 0.42 & 0.421 &  0.16 & -0.23 & 0.56 & 0.71 & 0.79 & 0.81 & 0.85 & \icc{0.740} & 0.496 & 0.876 \\
& Mastery               & 3     & 5.53 (1.02) & 5.56 (1.00) & 0.17 & 0.64 &  -0.03 & 0.19 & -0.42 & 0.37 & 0.890 & -0.03 & -0.42 & 0.36 & 0.79 & 0.79 & 0.72 & 0.76 & \icc{0.566} & 0.221 & 0.784 \\
& Meaning               & 3     & 4.99 (1.35) & 5.04 (1.30) & 0.13 & 0.45 &  -0.05 & 0.13 & -0.32 & 0.22 & 0.689 & -0.08 & -0.47 & 0.31 & 0.96 & 0.96 & 0.92 & 0.92 & \icc{0.881} & 0.749 & 0.946 \\
& Enjoyment             & 3     & 5.96 (0.85) & 6.07 (0.67) & 0.11 & 0.43 &  -0.11 & 0.13 & -0.37 & 0.16 & 0.415 & -0.17 & -0.56 & 0.23 & 0.94 & 0.94 & 0.86 & 0.88 & \icc{0.649} & 0.351 & 0.828 \\

\midrule
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{PENS}}}}
& Competence            & 3     & 5.57 (1.13) & 5.48 (1.24) & 0.22 & 0.92 &   0.09 & 0.25 & -0.42 & 0.60 & 0.709 &  0.08 & -0.32 & 0.47 & 0.85 & 0.86 & 0.93 & 0.94 & \icc{0.470} & 0.093 & 0.727 \\
& Autonomy              & 3     & 4.20 (1.45) & 4.37 (1.70) & 0.29 & 0.92 &  -0.17 & 0.25 & -0.69 & 0.34 & 0.493 & -0.14 & -0.53 & 0.26 & 0.80 & 0.82 & 0.89 & 0.89 & \icc{0.695} & 0.422 & 0.853 \\
& Relatedness           & 3     & 2.88 (1.53) & 2.91 (1.65) & 0.43 & 0.99 &  -0.03 & 0.25 & -0.55 & 0.50 & 0.917 & -0.02 & -0.41 & 0.37 & 0.77 & 0.78 & 0.81 & 0.85 & \icc{0.689} & 0.407 & 0.851 \\
& Presence/Immersion    & 8     & 3.37 (1.32) & 3.36 (1.39) & 0.29 & 0.76 &   0.01 & 0.20 & -0.40 & 0.42 & 0.965 &  0.01 & -0.38 & 0.40 & 0.88 & 0.89 & 0.92 & 0.92 & \icc{0.734} & 0.480 & 0.874 \\
& Intuitive Controls    & 3     & 6.17 (0.77) & 6.03 (1.18) & 0.14 & 0.60 &   0.15 & 0.18 & -0.23 & 0.52 & 0.427 &  0.16 & -0.23 & 0.55 & 0.66 & 0.74 & 0.87 & 0.91 & \icc{0.589} & 0.262 & 0.795 \\

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{GEQ}}}}
& Absorption            & 5     & 2.32 (0.89) & 2.33 (0.73) & 0.19 & 0.33 &  -0.01 & 0.09 & -0.20 & 0.18 & 0.931 & -0.02 & -0.41 & 0.37 & 0.81 & 0.82 & 0.77 & 0.77 & \icc{0.848} & 0.684 & 0.930 \\
& Flow                  & 9     & 2.60 (0.73) & 2.66 (0.74) & 0.15 & 0.31 &  -0.06 & 0.08 & -0.22 & 0.11 & 0.479 & -0.14 & -0.54 & 0.25 & 0.79 & 0.80 & 0.82 & 0.83 & \icc{0.852} & 0.695 & 0.932 \\
& Presence              & 4     & 2.98 (0.96) & 2.86 (0.94) & 0.22 & 0.50 &  0.12 & 0.13 & -0.15 & 0.39 & 0.365 &  0.18 & -0.21 & 0.58 & 0.66 & 0.70 & 0.76 & 0.79 & \icc{0.765} & 0.540 & 0.889 \\
& Immersion             & 1     & 3.44 (1.19) & 3.52 (1.23) & 0.25 & 0.56 &  -0.08 & 0.17 & -0.44 & 0.28 & 0.647 & -0.09 & -0.48 & 0.30 & -    & -    & -    & -    & \icc{0.753} & 0.514 & 0.883 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{AD}}}}
& Attractiveness        & 7     & 5.44 (1.01) & 5.39 (1.00) & 0.13 & 0.51 &   0.05 & 0.14 & -0.25 & 0.34 & 0.753 &  0.06 & -0.33 & 0.46 & 0.91 & 0.91 & 0.91 & 0.92 & \icc{0.750} & 0.508 & 0.882 \\
& HQ- identification    & 7     & 4.45 (0.79) & 4.39 (0.98) & 0.12 & 0.43 &   0.06 & 0.11 & -0.17 & 0.29 & 0.610 &  0.10 & -0.29 & 0.50 & 0.73 & 0.74 & 0.82 & 0.83 & \icc{0.811} & 0.617 & 0.912 \\
& HQ - stimulation      & 7     & 4.50 (0.98) & 4.53 (1.05) & 0.12 & 0.47 &  -0.02 & 0.11 & -0.25 & 0.21 & 0.840 & -0.04 & -0.43 & 0.35 & 0.82 & 0.84 & 0.84 & 0.85 & \icc{0.853} & 0.694 & 0.932 \\
& Pragmatic Quality     &       & 4.94 (0.87) & 4.80 (0.70) & 0.12 & 0.48 &   0.14 & 0.12 & -0.11 & 0.38 & 0.261 &  0.23 & -0.17 & 0.63 & 0.71 & 0.79 & 0.57 & 0.59 & \icc{0.715} & 0.457 & 0.862 \\
\bottomrule

\end{tabularx}
\begin{flushleft}
\footnotesize{$n=100$ for \emph{miniPXI}, \emph{NPS}, and appreciation; $n=25$ in all other cases, HQ = hedonic quality.}
\end{flushleft}
\end{table}
\end{landscape}
}

==> table_simplified.tex <==
\begin{table}
\centering
\caption{Mean and standard deviations ($SD$) across Week 1 and 3, Intra-class correlation coefficient (ICC) interpretation in terms of test-retest reliability (%ICC<0.25: very poor = \textcolor{cVpoor}{\rule{2.5ex}{1.5ex}}; 
$0.25 \leq ICC < 0.5$: poor = \textcolor{cPoor}{\rule{2.5ex}{1.5ex}}; $0.5 \leq ICC < 0.75$: moderate = \textcolor{cModerate}{\rule{2.5ex}{1.5ex}}; $0.75 \leq ICC < 0.9$: good = \textcolor{cGood}{\rule{2.5ex}{1.5ex}}; $ICC \geq 0.9$: excellent = \textcolor{cExcellent}{\rule{2.5ex}{1.5ex}}), 95\% confidence interval (CI), reliability analysis (Cronbach’s $\alpha$, and McDonald’s $\omega$) for multi-item measures across Week 1 and 3, for each construct.}
\label{table:all_questionnaires}
\begin{tabularx}{1.0\linewidth}{ll@{\hskip12pt} cc@{\hskip12pt} c@{\hskip12pt} cc@{\hskip12pt} cc@{\hskip15pt} cc}
    \toprule
     &  &  &  &    &  &  & \multicolumn{4}{c}{\hskip-5pt\textbf{Internal Consistency}} \\
     &  & \multicolumn{2}{c}{\hskip-15pt\textbf{Mean ($SD$)}}   &  & \multicolumn{2}{c}{\hskip-15pt\textbf{95\% CI}} & \multicolumn{2}{c}{\hskip-15pt\textbf{Week 1}} & \multicolumn{2}{c}{\hskip-5pt\textbf{Week 3}} \\
     & \textbf{Construct} & \textbf{Week 1} & \textbf{Week 2} & \textbf{ICC} & \textbf{Lower} & \textbf{Upper} & $\bm{\alpha}$ & $\bm{\omega}$ & $\bm{\alpha}$ & $\bm{\omega}$ \\
     \midrule
     \parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textbf{miniPXI}}}} 
     & Audiovisual Appeal \textit{(1 item)}  & 5.65 (1.35) & 5.69 (1.35) &  \icc{.630} & 0.496 & 0.735 & -    & -    & -    & -    \\
     & Challenge \textit{(1 item)}           & 4.80 (1.51) & 5.12 (1.53) &  \icc{.422} & 0.249 & 0.570 & -    & -    & -    & -    \\
     & Ease of Control \textit{(1 item)}     & 6.01 (1.38) & 6.06 (1.16) &  \icc{.479} & 0.312 & 0.617 & -    & -    & -    & -    \\
     & Clarity of Goals \textit{(1 item)}    & 5.72 (1.61) & 5.77 (1.51) &  \icc{.624} & 0.488 & 0.731 & -    & -    & -    & -    \\
     & Progress Feedback \textit{(1 item)}   & 5.11 (1.61) & 5.00 (1.75) &  \icc{.651} & 0.522 & 0.751 & -    & -    & -    & -    \\
     & Autonomy \textit{(1 item) }          & 5.32 (1.50) & 5.12 (1.47) &  \icc{.505} & 0.345 & 0.637 & -    & -    & -    & -    \\
     & Curiosity \textit{(1 item)  }        & 5.64 (1.24) & 5.69 (1.40) &  \icc{.547} & 0.393 & 0.671 & -    & -    & -    & -    \\
     & Immersion \textit{(1 item)   }       & 6.19 (1.10) & 6.07 (1.17) &  \icc{.365} & 0.183 & 0.523 & -    & -    & -    & -    \\
     & Mastery \textit{(1 item)    }        & 5.43 (1.43) & 5.43 (1.22) &  \icc{.447} & 0.274 & 0.591 & -    & -    & -    & -    \\
     & Meaning \textit{(1 item)  }          & 4.72 (1.49) & 4.72 (1.53) &  \icc{.644} & 0.513 & 0.746 & -    & -    & -    & -    \\
     & Enjoyment \textit{(1 item)  }        & 5.88 (1.24) & 5.88 (1.26) &  \icc{.704} & 0.590 & 0.791 & -    & -    & -    & -    \\
     \midrule
     \multicolumn{2}{l}{\textbf{NPS} \textit{(1 item)}} & 6.21 (2.65) & 6.29 (2.74) & \icc{.791} & 0.704 & 0.854 & -    & -    & -    & -    \\
     \midrule
     \multicolumn{2}{l}{\textbf{Appreciation} \textit{(1 item)}} & 5.70 (1.28) & 5.73 (1.25) & \icc{.795} & 0.710 & 0.857 & -    & -    & -    & -    \\
     \midrule
     \parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textbf{PXI}}}}
     & Audiovisual Appeal (\textit{3 items) }  & 5.92 (1.00) & 5.92 (0.90) & \icc{.668} & 0.374 & 0.840 & 0.95 & 0.96 & 0.94 & 0.94 \\
     & Challenge \textit{(3 items) }           & 5.12 (1.37) & 5.03 (1.23) & \icc{.820} & 0.634 & 0.916 & 0.88 & 0.88 & 0.8  & 0.81 \\
     & Ease of Control \textit{(3 items)   }   & 6.08 (1.00) & 6.20 (0.71) & \icc{.643} & 0.341 & 0.825 & 0.90 & 0.91 & 0.78 & 0.81 \\
     & Clarity of Goals \textit{(3 items) }    & 5.88 (1.03) & 5.72 (1.01) & \icc{.856} & 0.701 & 0.934 & 0.89 & 0.90 & 0.89 & 0.89 \\
     & Progress Feedback \textit{(3 items) }   & 5.41 (1.26) & 5.53 (1.48) & \icc{.664} & 0.370 & 0.837 & 0.88 & 0.89 & 0.90 & 0.90 \\
     & Autonomy \textit{(3 items) }          & 5.05 (1.37) & 5.04 (1.32) & \icc{.657} & 0.356 & 0.833 & 0.91 & 0.91 & 0.91 & 0.91 \\
     & Curiosity (\textit{3 items)  }         & 6.04 (0.67) & 5.87 (1.07) & \icc{.495} & 0.137 & 0.740 & 0.90 & 0.91 & 0.94 & 0.94 \\
     & Immersion \textit{(3 items)  }        & 5.77 (0.87) & 5.65 (1.13) & \icc{.740} & 0.496 & 0.876 & 0.71 & 0.79 & 0.81 & 0.85 \\
     & Mastery \textit{(3 items)  }           & 5.53 (1.02) & 5.56 (1.00) & \icc{.566} & 0.221 & 0.784 & 0.79 & 0.79 & 0.72 & 0.76 \\
     & Meaning \textit{(3 items) }            & 4.99 (1.35) & 5.04 (1.30) & \icc{.881} & 0.749 & 0.946 & 0.96 & 0.96 & 0.92 & 0.92 \\
     & Enjoyment \textit{(3 items)  }         & 5.96 (0.85) & 6.07 (0.67) & \icc{.649} & 0.351 & 0.828 & 0.94 & 0.94 & 0.86 & 0.88 \\
     \midrule
     \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{PENS}}}}
     & Competence \textit{(3 items) }          & 5.57 (1.13) & 5.48 (1.24) & \icc{.470} & 0.093 & 0.727 & 0.85 & 0.86 & 0.93 & 0.94 \\
     & Autonomy \textit{(3 items) }           & 4.20 (1.45) & 4.37 (1.70) & \icc{.695} & 0.422 & 0.853 & 0.80 & 0.82 & 0.89 & 0.89 \\
     & Relatedness  \textit{(3 items)  }      & 2.88 (1.53) & 2.91 (1.65) & \icc{.689} & 0.407 & 0.851 & 0.77 & 0.78 & 0.81 & 0.85 \\
     & Presence/Immersion \textit{(8 items)}  & 3.37 (1.32) & 3.36 (1.39) & \icc{.734} & 0.480 & 0.874 & 0.88 & 0.89 & 0.92 & 0.92 \\
     & Intuitive Controls \textit{(3 items) } & 6.17 (0.77) & 6.03 (1.18) & \icc{.589} & 0.262 & 0.795 & 0.66 & 0.74 & 0.87 & 0.91 \\
     \midrule
     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{GEQ}}}}
     & Absorption \textit{(5 items)  }        & 2.32 (0.89) & 2.33 (0.73) & \icc{.848} & 0.684 & 0.930 & 0.81 & 0.82 & 0.77 & 0.77 \\
     & Flow  \textit{(9 items)  }             & 2.60 (0.73) & 2.66 (0.74) & \icc{.852} & 0.695 & 0.932 & 0.79 & 0.80 & 0.82 & 0.83 \\
     & Presence \textit{(4 items)}           & 2.98 (0.96) & 2.86 (0.94) & \icc{.765} & 0.540 & 0.889 & 0.66 & 0.70 & 0.76 & 0.79 \\
     & Immersion \textit{(1 item)  }       & 3.44 (1.19) & 3.52 (1.23) & \icc{.753} & 0.514 & 0.883 & -    & -    & -    & -    \\
     \midrule
     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{AD}}}}
     & Attractiveness  \textit{ (7 items) }    & 5.44 (1.01) & 5.39 (1.00) & \icc{.750} & 0.508 & 0.882 & 0.91 & 0.91 & 0.91 & 0.92 \\
     & HQ - Identification \textit{(7 items) } & 4.45 (0.79) & 4.39 (0.98) & \icc{.811} & 0.617 & 0.912 & 0.73 & 0.74 & 0.82 & 0.83 \\
     & HQ - Stimulation \textit{(7 items) }    & 4.50 (0.98) & 4.53 (1.05) & \icc{.853} & 0.694 & 0.932 & 0.82 & 0.84 & 0.84 & 0.85 \\
     & Pragmatic Quality \textit{(7 items)  } & 4.94 (0.87) & 4.80 (0.70) & \icc{.715} & 0.457 & 0.862 & 0.71 & 0.79 & 0.57 & 0.59 \\
     \bottomrule
\end{tabularx}
\begin{flushleft}
\footnotesize{$n=100$ for miniPXI, NPS, and appreciation; $n=25$ in all other cases, HQ = hedonic quality.}
\end{flushleft}
\end{table}
